Duckiefloat: a Collision-Tolerant Resource-Constrained Blimp for Long-Term Autonomy in Subterranean Environments

There are several challenges for search and rescue robots: mobility, perception, autonomy, and communication. Inspired by the DARPA Subterranean (SubT) Challenge, we propose an autonomous blimp robot, which has the advantages of low power consumption and collision-tolerance compared to other aerial vehicles like drones. This is important for search and rescue tasks that usually last for one or more hours. However, the underground constrained passages limit the size of blimp envelope and its payload, making the proposed system resource-constrained. Therefore, a careful design consideration is needed to build a blimp system with on-board artifact search and SLAM. In order to reach long-term operation, a failure-aware algorithm with minimal communication to human supervisor to have situational awareness and send control signals to the blimp when needed.

==> 03A_requirements.tex <==



==> lamacro.tex <==
\def\cstart{\cslidebegin{} \cslidenotitle \vfill \small }
\def\cend{\vfill\cslideend}
\def\add{\addtolength}
\def\addpar{\addtolength{\parskip}}

%\newlength{\yfigsize}
%\newlength{\xfigsize}
%\newlength{\figsize}
%\setlength{\yfigsize}{5.0truein}
%\setlength{\xfigsize}{3.3truein}
%\newfont{\tenssbx}{cmssbx10}
%\newfont{\twelvessbx}{cmssbx10 scaled \magstep1}
%\newfont{\fourteenssbx}{cmssbx10 scaled \magstep2}
%\newfont{\sixteenssbx}{cmssbx10 scaled \magstep3}

\newcommand{\bbull}{\begin{tabbing} \hspace{0.25in}\= \kill}
\newcommand{\ebull}{\end{tabbing}}
\newcommand{\bull}{$\bullet$ \> }
\newcommand{\btab}{ \> }

% This typesets a paragraph consisting of #1, dot leaders, and then #2
% flush to the right margin.  It is used for index and table of contents
% entries.  The paragraph is indented by \leftskip.
% 
\def\entry #1#2{\begingroup
  %
  % Start a new paragraph if necessary, so our assignments below can't
  % affect previous text.
  \par
  %
  % Do not fill out the last line with white space.
  \parfillskip = 0in
  %
  % No extra space above this paragraph.
  \parskip = 0in
  %
  % Do not prefer a separate line ending with a hyphen to fewer lines.
  \finalhyphendemerits = 0
  %
  % \hangindent is only relevant when the entry text and page number
  % don't both fit on one line.  In that case, bob suggests starting the
  % dots pretty far over on the line.  Unfortunately, a large
  % indentation looks wrong when the entry text itself is broken across
  % lines.  So we use a small indentation and put up with long leaders.
  % 
  % \hangafter is reset to 1 (which is the value we want) at the start
  % of each paragraph, so we need not do anything with that.
  \hangindent=2em
  %
  % When the entry text needs to be broken, just fill out the first line
  % with blank space.
  \rightskip = 0pt plus1fil
  %
  % Start a ``paragraph'' for the index entry so the line breaking
  % parameters we've set above will have an effect.
  \noindent
  %
  % Insert the text of the index entry.  TeX will do line-breaking on it.
  #1%
  %
  % If we must, put the page number on a line of its own, and fill out
  % this line with blank space.  (The \hfil is overwhelmed with the
  % fill leaders glue in \indexdotfill if the page number does fit.)
  \hfil\penalty50
  \null\nobreak\indexdotfill % Have leaders before the page number.
  %
  % The `\ ' here is removed by the implicit \unskip that TeX does as
  % part of (the primitive) \par.  Without it, a spurious underfull
  % \hbox ensues.
  \ #2% The page number ends the paragraph.
  \par
\endgroup}

% Like \dotfill except takes at least 1 em.
\def\indexdotfill{\cleaders
  \hbox{$\mathsurround=0pt \mkern1.5mu . \mkern1.5mu$}\hskip 1em plus 1fill}
%\setlength{\textwidth}{6.5truein}
%\setlength{\textheight}{9.0truein}

%\newcommand{\ifundefined}[2]{\expandafter\ifx\csname#1\endcsname\relax\else
%  \expandafter\gdef\csname#1\endcsname{#2} \fi}

%\newcommand{\hrule}{\rule{\thetextwidth}{.02mm}}

%\newcommand{\qed}{\noindent$\Box$}
%\def\qed{$\fbox{\phantom{\tiny c}}$\bigskip\par}
\def\qed{$\blacksquare$}
\def\brack#1{\left( {#1} \right)}
\def\sqbrack#1{\left[ {#1} \right]}
\def\curbrack#1{\left\{ {#1} \right\}}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\ba}{\begin{eqnarray*}}
\newcommand{\ea}{\end{eqnarray*}}
\newcommand{\bal}{\begin{align*}}
\newcommand{\eal}{\end{align*}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\def\bs{\begin{slide}{}}
\def\es{\end{slide}{}}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\newcommand{\barr}{\begin{array}}
\newcommand{\earr}{\end{array}}
\newcommand{\lamatrix}{\left[ \begin{array}}
\newcommand{\elamatrix}{\end{array}\right]}
\newcommand{\ma}{\left[ \begin{array}}
\newcommand{\ema}{\end{array}\right]}
\newcommand{\ssparam}[9]{
\left[ \begin{array}{c|cc}
#1 & #2 & #3 \\
\hline
#4 & #5 & #6 \\
#7 & #8 & #9 
\end{array}
\right]
}
\newcommand{\ULine}[1]{$\underline{\mbox{#1}}$}
\newcommand{\Uline}[1]{$\underline{\mbox{#1}}$}
\renewcommand\exp[1]{ e^{{#1}} }

\newtheorem{theo}{Theorem}
%\newtheorem{algorithm}{Algorithm}
%\newtheorem{fact}{Fact}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
% \newtheorem{result}{Result}
% \newtheorem{definition}{Definition}
% \newtheorem{example}{Example}
\newtheorem{remark}{Remark}

%\def\proof{\par\noindent{\bf Proof: }}

\newcommand{\lineeqn}[1]{(\ref{#1})}
\newcommand{\bracket}[1]{\left\{ {#1} \right\} }
\def\bcase{\left\{ \begin{array}{ll}} 
\def\ecase{\end{array} \right.}
\def\emptybegin{\cslidebegin{}\cslidenotitle\raggedright}
\def\th{^{th}}

\newcommand{\sq}{ ^2 }
\newcommand{\tr}{ ^T }
\def\diag{ {\rm diag} }
\renewcommand{\star}{ ^* }
\newcommand{\pinv}{ ^{\dagger} }
%\def\span{ {\rm span} }
\newcommand{\til}[1]{ {\widetilde{#1}} }
\newcommand{\inv}{ ^{-1} }
\newcommand{\invT}{ ^{-T} }
\newcommand{\roottwo}{ \sqrt{2} }
\newcommand{\half}{ {\frac{1}{2}} }
\newcommand{\adj}{ {^*} }
\newcommand{\by}{\times}
\newcommand{\tends}{\rightarrow}
\newcommand{\trace}{{\rm tr} }
\newcommand{\sigmamin}{ {\sigma}_{\min} }
\newcommand{\sgn}{ \mbox{sgn} }
\newcommand{\sat}{ \mbox{sat} }
\def\Lap#1{ \widehat{#1}(s) }

\newcommand{\calA}{ {\cal A} }
\newcommand{\order}{ {\cal O} }

%\newcommand{\dddot}[1]{ {\stackrel {...}{#1} } }
\newcommand{\Ltwo}{ {L_2} }
\def\Ltwoe{ {{L_2}_e} }
\newcommand{\innerpct}[2]{ \left<{#1},{#2}\right> }
\newcommand{\norm}[1]{\left\| {#1} \right\|}
\def\Hinfnorm#1{ \norm{ #1 }_{H_\infty} }
\newcommand{\abs}[1]{\left| {#1} \right|}
\newcommand{\summing}[3]{\sum_{{#1}={#2}}^{#3}}
\newcommand{\integral}[2]{\int_{#1}^{#2}}
\newcommand{\dd}[1]{\frac{d}{d{#1}}}
\newcommand{\pptwo}[2]{ \frac{\partial{#1}}{\partial{#2}} }
\newcommand{\ppthree}[3]{ \frac{\partial^{#3}{#1}}{\partial^{#3}{#2}}}
%\newcommand{\defeq}{ \stackrel{\Delta}{=} }
\def\defeq{:=}
\def\rr#1{\mathbb{R}^{#1}}
\newcommand{\rrsub}[1]{ \mathbb{R}_{#1} }

\newcommand{\nullsp}{ {\cal N} }
\newcommand{\rangesp}{ {\cal R} }
\newcommand{\orthsum}{ \stackrel{\perp}{\oplus} }
\newcommand{\jw}{ {j \omega} }
\def\rad{ \mbox{rad}}
\def\meter{ \mbox{m}}
\def\sec{\mbox{sec}}
\def\plus{^{+}}
\def\minus{^{-}}
\def\grad{\nabla}

\font\teeny = cmss10 scaled \magstep 1
%\newcommand{\cirsse}{\footnotetext{\vspace{-0.70in} 
%               \teeny \today\ \  (jtw) \hfill\rule[0.08in]{3.6in}{0.01in}
%               \hspace{-0.05in}CIRSSE\rule[0.08in]{0.25in}{0.01in}
%}}

\def\cirsse{\footnotetext{\vspace{-0.70in} \teeny \today \ \ 
(JTW)\hfill\rule[0.08in]{3.6in}{0.01in}  
\special{psfile = /home/wen/tex/cirsse.ps1 hscale= 0.275 vscale= 0.275
hoffset=-0.585 voffset= -2.81} 
}}
\def\cirssedate#1{\footnotetext{\vspace{-0.70in} \teeny {#1} \ \ 
(JTW)\hfill\rule[0.08in]{3.6in}{0.01in}  
\special{psfile = /home/wen/tex/cirsse.ps1 hscale= 0.275 vscale= 0.275
hoffset=-0.585 voffset= -2.81} 
}}

\newcommand{\cat}{\footnotetext{\vspace{-0.70in} 
                \teeny \today (jtw) \hfill\rule[0.08in]{4in}{0.01in}
                \hspace{-0.05in}CAT\rule[0.08in]{0.25in}{0.01in}  }}

\newcommand{\comments}[1]{}

\def\clamup{C\kern.1667em\lower-.5ex\hbox{La}\kern.125emMS\ }
\def\clamdown{C\kern-.1667em\lower.5ex\hbox{La}\kern-.125emMS\ }

\def\stitle#1{ {\leftline{ #1}}}
\def\bftitle#1{ {\leftline{\bf #1}}}
\def\suline#1{ {\leftline{\Uline{{#1}}}}}

\def\topline{\rule[.15in]{6.35in}{0.070in}\vspace{-0.3cm}\newline}
\def\lowline{\par\vspace{-1.5cm}\rule[-.10in]{6.35in}{.070in}
        \par}
\def\shead#1{\topline\bc{#1}\ec\lowline\raggedright\medskip}
\def\rpi{ {Rensselaer Polytechnic Institute} }

% Local Variables: 
% mode: latex
% TeX-master: t
% End:
